Boosting background suppression in the NEXT experiment through Richardson-Lucy deconvolution

Next-generation neutrinoless double beta decay experiments aim for half-life sensitivities of ~$10^{27}$ yr, requiring suppressing backgrounds to <1 count/tonne/yr. For this, any extra background rejection handle, beyond excellent energy resolution and the use of extremely radiopure materials, is of utmost importance. The NEXT experiment exploits differences in the spatial ionization patterns of double beta decay and single-electron events to discriminate signal from background. While the former display two Bragg peak dense ionization regions at the opposite ends of the track, the latter typically have only one such feature. Thus, comparing the energies at the track extremes provides an additional rejection tool. The unique combination of the topology-based background discrimination and excellent energy resolution (1% FWHM at the Q-value of the decay) is the distinguishing feature of NEXT. Previous studies demonstrated a topological background rejection factor of ~5 when reconstructing electron-positron pairs in the $^{208}$Tl 1.6 MeV double escape peak (with Compton events as background), recorded in the NEXT-White demonstrator at the Laboratorio Subterr\'aneo de Canfranc, with 72% signal efficiency. This was recently improved through the use of a deep convolutional neural network to yield a background rejection factor of ~10 with 65% signal efficiency. Here, we present a new reconstruction method, based on the Richardson-Lucy deconvolution algorithm, which allows reversing the blurring induced by electron diffusion and electroluminescence light production in the NEXT TPC. The new method yields highly refined 3D images of reconstructed events, and, as a result, significantly improves the topological background discrimination. When applied to real-data 1.6 MeV $e^-e^+$ pairs, it leads to a background rejection factor of 27 at 57% signal efficiency.

==> src/Authors_from_Justo.tex <==
\collaboration{The NEXT Collaboration}
%
\author[6,a]{A.~Sim\'on, \note[a]{Corresponding author.}}
%
\author[6,7]{Y.~Ifergan,}
%
\author[6]{A.B.~Redwine,}
%
\author[6,b]{R.~Weiss-Babai,\note[b]{Now in Soreq Nuclear Research Center, Yavneh, Israel.}}
%
\author[6,c]{L.~Arazi, \note[c]{Corresponding author.}}
%
\author[20]{C.~Adams,}
%
\author[25]{V.~\'Alvarez,}
%
\author[6]{L.~Arazi,}
%
\author[23]{I.J.~Arnquist,}
%
\author[4]{C.D.R~Azevedo,}
%
\author[20]{K.~Bailey,}
%
\author[25]{F.~Ballester,}
%
\author[17]{J.M.~Benlloch-Rodr\'{i}guez,}
%
\author[14]{F.I.G.M.~Borges,}
%
\author[3]{N.~Byrnes,}
%
\author[22]{S.~C\'arcel,}
%
\author[22]{J.V.~Carri\'on,}
%
\author[26]{S.~Cebri\'an,}
%
\author[23]{E.~Church,}
%
\author[14]{C.A.N.~Conde,}
%
\author[11]{T.~Contreras,}
%
\author[2]{A.A.~Denisenko,}
%
\author[24]{G.~D\'iaz,}
%
\author[22]{J.~D\'iaz,}
%
\author[14]{J.~Escada,}
%
\author[25]{R.~Esteve,}
%
\author[6,22]{R.~Felkai,}
%
\author[13]{L.M.P.~Fernandes,}
%
\author[9,17]{P.~Ferrario,}
%
\author[4]{A.L.~Ferreira,}
%
\author[2]{F.~Foss,}
%
\author[13]{E.D.C.~Freitas,}
%
\author[9,18]{Z.~Freixa,}
%
\author[17]{J.~Generowicz,}
%
\author[8]{A.~Goldschmidt,}
%
\author[9,17,a]{J.J.~G\'omez-Cadenas,\note[a]{NEXT Co-spokesperson.}}
%
\author[17]{R.~Gonz\'alez,}
%
\author[24]{D.~Gonz\'alez-D\'iaz,}
%
\author[11]{S.~Gosh,}
%
\author[11]{R.~Guenette,}
%
\author[10]{R.M.~Guti\'errez,}
%
\author[11]{J.~Haefner,}
%
\author[20]{K.~Hafidi,}
%
\author[1]{J.~Hauptman,}
%
\author[13]{C.A.O.~Henriques,}
%
\author[24]{J.A.~Hernando~Morata,}
%
\author[17]{P.~Herrero,}
%
\author[25]{V.~Herrero,}
%
\author[11]{J.~Ho,}
%
\author[6,7]{Y.~Ifergan,}
%
\author[3]{B.J.P.~Jones,}
%
\author[24]{M.~Kekic,}
%
\author[21]{L.~Labarga,}
%
\author[3]{A.~Laing,}
%
\author[5]{P.~Lebrun,}
%
\author[22]{N.~L\'opez-March,}
%
\author[10]{M.~Losada,}
%
\author[13]{R.D.P.~Mano,}
%
\author[11,22]{J.~Mart\'in-Albo,}
%
\author[22]{A.~Mart\'inez,}
%
\author[17,22]{M.~Mart\'inez-Vara,}
%
\author[6]{G.~Mart\'inez-Lema,}
%
\author[3]{A.D.~McDonald,}
%
\author[20]{Z.E.~Meziani,}
%
\author[9,17]{F.~Monrabal,}
%
\author[13]{C.M.B.~Monteiro,}
%
\author[25]{F.J.~Mora,}
%
\author[22]{J.~Mu\~noz Vidal,}
%
\author[2]{C.~Newhouse,}
%
\author[22]{P.~Novella,}
%
\author[3,a]{D.R.~Nygren,}
%
\author[17]{E.~Oblak,}
%
\author[22,24]{B.~Palmeiro,}
%
\author[5]{A.~Para,}
%
\author[12]{J.~P\'erez,}
%
\author[23]{M.~Querol,}
%
\author[5]{A.~Redwine,}
%
\author[23]{J.~Renner,}
%
\author[19]{L.~Ripoll,}
%
\author[9,17]{I.~Rivilla,}
%
\author[10]{Y.~Rodr\'iguez Garc\'ia,}
%
\author[25]{J.~Rodr\'iguez,}
%
\author[16]{C.~Rogero,}
%
\author[3]{L.~Rogers,}
%
\author[12,17]{B.~Romeo,}
%
\author[22]{C.~Romo-Luque,}
%
\author[14]{F.P.~Santos,}
%
\author[13]{J.M.F.~dos~Santos,}
%
\author[6]{A.~Sim\'on,}
%
\author[22]{M.~Sorel,}
%
\author[11]{C.~Stanford,}
%
\author[13]{J.M.R.~Teixeira,}
%
\author[2]{P.~Thapa}
%
\author[25]{J.F.~Toledo,}
%
\author[17]{J.~Torrent,}
%
\author[22]{A.~Us\'on,}
%
\author[4]{J.F.C.A.~Veloso,}
%
\author[2]{T.T.~Vuong,}
%
\author[15]{R.~Webb,}
%
\author[6,b]{R.~Weiss-Babai,\note[b]{Now at Soreq Nuclear Research Center, Yavneh, Israel.}}
%
\author[15,c]{J.T.~White,\note[c]{Deceased.}}
%
\author[3]{K.~Woodruff,}
%
\author[22]{N.~Yahlali}
%
\affiliation[1]{
Department of Physics and Astronomy, Iowa State University, Ames, Iowa, USA}
%
\affiliation[2]{
Department of Chemistry and Biochemistry, University of Texas at Arlington, Arlington, Texas, USA}
%
\affiliation[3]{
Department of Physics, University of Texas at Arlington, Arlington, Texas, USA}
%
\affiliation[4]{
Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro, Aveiro, Portugal}
%
\affiliation[5]{
Fermi National Accelerator Laboratory, Batavia, Illinois, USA}
%
\affiliation[6]{
Unit of Nuclear Engineering, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, Beer-Sheva, Israel}
%
\affiliation[7]{
Nuclear Research Center Negev, Beer-Sheva, Israel}
%
\affiliation[8]{
Lawrence Berkeley National Laboratory, Berkeley, California, USA}
%
\affiliation[9]{
Ikerbasque (Basque Foundation for Science), Bilbao, Spain}
%
\affiliation[10]{
Centro de Investigaci\'on en Ciencias B\'asicas y Aplicadas, Universidad Antonio Nari\~no, Bogot\'a, Colombia}
%
\affiliation[11]{
Department of Physics, Harvard University, Cambridge, Massachusetts, USA}
%
\affiliation[12]{
Laboratorio Subterr\'aneo de Canfranc, Canfranc-Estaci\'on, Spain}
%
\affiliation[13]{
LIBPhys, Universidade de Coimbra, Coimbra, Portugal}
%
\affiliation[14]{
LIP, Departamento de Física, Universidade de Coimbra, Coimbra, Portugal}
%
\affiliation[15]{
Department of Physics and Astronomy, Texas A\&M University, College Station, Texas, USA}
%
\affiliation[16]{
Centro de F\'isica de Materiales (CFM), CSIC \& Universidad del Pa\'is Vasco (UPV/EHU), Donostia-San Sebasti\'an, Spain}
%
\affiliation[17]{
Donostia International Physics Center (DIPC), Donostia-San Sebasti\'an, Spain}
%
\affiliation[18]{
Departmento de Qu\'imica Org\'anica I, Universidad del Pa\'is Vasco (UPV/EHU), Donostia-San Sebasti\'an, Spain}
%
\affiliation[19]{
Escola Polit\`ecnica Superior, Universitat de Girona, Girona, Spain}
%
\affiliation[20]{
Argonne National Laboratory, Lemont, Illinois, USA}
%
\affiliation[21]{
Departamento de F\'isica Te\'orica, Universidad Aut\'onoma de Madrid, Madrid, Spain}
%
\affiliation[22]{
Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Paterna, Spain}
%
\affiliation[23]{
Pacific Northwest National Laboratory, Richland, Washington, USA}
%
\affiliation[24]{
Instituto Gallego de F\'isica de Altas Energ\'ias, Universidade de Santiago de Compostela, Santiago de Compostela, Spain}
%
\affiliation[25]{
Instituto de Instrumentaci\'on para Imagen Molecular (I3M), CSIC \& Univ.\ Polit\`ecnica de Val\`encia, Valencia, Spain}
%
\affiliation[26]{
Centro de Astropart\'iculas y F\'isica de Altas Energ\'ias (CAPA), Universidad de Zaragoza, Zaragoza, Spain}
%
\emailAdd{next-src@pegaso.ific.uv.es}


==> src/authors2.tex <==
\collaboration{The NEXT Collaboration}
%
\author[6,a]{A.~Sim\'on, \note[a]{Corresponding author.}}
%
\author[6,7]{Y.~Ifergan,}
%
\author[6]{A.B.~Redwine,}
%
\author[6,b]{R.~Weiss-Babai,\note[b]{Now in Soreq Nuclear Research Center, Yavneh, Israel.}}
%
\author[6,c]{L.~Arazi, \note[c]{Corresponding author.}}
%
\author[2]{C.~Adams,}
%
\author[16]{H.~Almaz\'an,}
%
\author[22]{V.~\'Alvarez,}
%
\author[24]{B.~Aparicio,}
%
\author[24]{A.I.~Aranburu,}
%
\author[20]{I.J.~Arnquist,}
%
\author[4]{C.D.R~Azevedo,}
%
\author[2]{K.~Bailey,}
%
\author[22]{F.~Ballester,}
%
\author[16,19]{J.M.~Benlloch-Rodr\'{i}guez,}
%
\author[14]{F.I.G.M.~Borges,}
%
\author[3]{N.~Byrnes,}
%
\author[19]{S.~C\'arcel,}
%
\author[19]{J.V.~Carri\'on,}
%
\author[23]{S.~Cebri\'an,}
%
\author[20]{E.~Church,}
%
\author[14]{C.A.N.~Conde,}
%
\author[11]{T.~Contreras,}
%
\author[24,9]{F.P.~Coss\'io,}
%
\author[26]{A.A.~Denisenko,}
%
\author[21]{G.~D\'iaz,}
%
\author[19]{J.~D\'iaz,}
%
\author[5]{M.~Diesburg,}
%
\author[14]{J.~Escada,}
%
\author[22]{R.~Esteve,}
%
\author[6,7,19]{R.~Felkai,}
%
\author[13]{L.M.P.~Fernandes,}
%
\author[16,9]{P.~Ferrario,}
%
\author[4]{A.L.~Ferreira,}
%
\author[13]{E.D.C.~Freitas,}
%
\author[24,9]{Z.~Freixa,}
%
\author[16]{J.~Generowicz,}
%
\author[11]{S.~Ghosh,}
%
\author[8]{A.~Goldschmidt,}
%
\author[16,9,d]{J.J.~G\'omez-Cadenas,\note[d]{NEXT Co-spokesperson.}}
%
\author[16]{R.~Gonz\'alez,}
%
\author[21]{D.~Gonz\'alez-D\'iaz,}
%
\author[11]{R.~Guenette,}
%
\author[10]{R.M.~Guti\'errez,}
%
\author[11]{J.~Haefner,}
%
\author[2]{K.~Hafidi,}
%
\author[1]{J.~Hauptman,}
%
\author[13]{C.A.O.~Henriques,}
%
\author[21]{J.A.~Hernando~Morata,}
%
\author[16,25]{P.~Herrero,}
%
\author[22]{V.~Herrero,}
%
\author[11]{J.~Ho,}
%
\author[3]{B.J.P.~Jones,}
%
\author[21,19]{M.~Kekic,}
%
\author[18]{L.~Labarga,}
%
\author[3]{A.~Laing,}
%
\author[5]{P.~Lebrun,}
%
\author[22,19]{N.~L\'opez-March,}
%
\author[10]{M.~Losada,}
%
\author[13]{R.D.P.~Mano,}
%
\author[19]{J.~Mart\'in-Albo,}
%
\author[19,16]{A.~Mart\'inez,}
%
\author[19]{M.~Mart\'inez-Vara,}
%
\author[19,21,e]{G.~Mart\'inez-Lema,\note[e]{Now at the Unit of Nuclear Engineering, Ben-Gurion University, Beer-Sheva, Israel.}}
%
\author[3]{A.D.~McDonald,}
%
\author[2]{Z.-E.~Meziani,}
%
\author[16,9]{F.~Monrabal,}
%
\author[13]{C.M.B.~Monteiro,}
%
\author[22]{F.J.~Mora,}
%
\author[19,16]{J.~Mu\~noz Vidal,}
%
\author[3]{K.~Navarro,}
%
\author[19]{P.~Novella,}
%
\author[3,f]{D.R.~Nygren,\note[f]{NEXT Co-spokesperson.}}
%
\author[16]{E.~Oblak,}
%
\author[16]{M.~Odriozola-Gimeno,}
%
\author[21,19]{B.~Palmeiro,}
%
\author[5]{A.~Para,}
%
\author[12]{J.~P\'erez,}
%
\author[19]{M.~Querol,}
%
\author[21,19]{J.~Renner,}
%
\author[17]{L.~Ripoll,}
%
\author[16,9]{I.~Rivilla,}
%
\author[10]{Y.~Rodr\'iguez Garc\'ia,}
%
\author[22]{J.~Rodr\'iguez,}
%
\author[25]{C.~Rogero,}
%
\author[3]{L.~Rogers,}
%
\author[16,12]{B.~Romeo,}
%
\author[19]{C.~Romo-Luque,}
%
\author[14]{F.P.~Santos,}
%
\author[13]{J.M.F. dos~Santos,}
%
\author[19]{M.~Sorel,}
%
\author[15,g]{C.~Sofka,\note[g]{Now at University of Texas at Austin, USA.}}
%
\author[11]{C.~Stanford,}
%
\author[15]{T.~Stiegler,}
%
\author[13]{J.M.R. Teixeira,}
%
\author[26]{P.~Thapa,}
%
\author[22]{J.F.~Toledo,}
%
\author[16]{J.~Torrent,}
%
\author[19]{A.~Us\'on,}
%
\author[4]{J.F.C.A.~Veloso,}
%
\author[15]{R.~Webb,}
%
\author[15,h]{J.T.~White,\note[h]{Deceased.}}
%
\author[3]{K.~Woodruff,}
%
\author[19]{N.~Yahlali}
%
\emailAdd{ander@post.bgu.ac.il}
\emailAdd{larazi@post.bgu.ac.il}
%
\affiliation[1]{
Department of Physics and Astronomy, Iowa State University, 12 Physics Hall, Ames, IA 50011-3160, USA}
%
\affiliation[2]{
Argonne National Laboratory, Argonne, IL 60439, USA}
%
\affiliation[3]{
Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\affiliation[4]{
Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro, Campus de Santiago, Aveiro, 3810-193, Portugal}
%
\affiliation[5]{
Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
%
\affiliation[6]{
Unit of Nuclear Engineering, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\affiliation[7]{
Nuclear Research Center Negev, Beer-Sheva, 84190, Israel}
%
\affiliation[8]{
Lawrence Berkeley National Laboratory (LBNL), 1 Cyclotron Road, Berkeley, CA 94720, USA}
%
\affiliation[9]{
Ikerbasque, Basque Foundation for Science, Bilbao, E-48013, Spain}
%
\affiliation[10]{
Centro de Investigaci\'on en Ciencias B\'asicas y Aplicadas, Universidad Antonio Nari\~no, Sede Circunvalar, Carretera 3 Este No.\ 47 A-15, Bogot\'a, Colombia}
%
\affiliation[11]{
Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\affiliation[12]{
Laboratorio Subterr\'aneo de Canfranc, Paseo de los Ayerbe s/n, Canfranc Estaci\'on, E-22880, Spain}
%
\affiliation[13]{
LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\affiliation[14]{
LIP, Department of Physics, University of Coimbra, Coimbra, 3004-516, Portugal}
%
\affiliation[15]{
Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843-4242, USA}
%
\affiliation[16]{
Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, 20018 San Sebastián / Donostia, Spain}
%
\affiliation[17]{
Escola Polit\`ecnica Superior, Universitat de Girona, Av.~Montilivi, s/n, Girona, E-17071, Spain}
%
\affiliation[18]{
Departamento de F\'isica Te\'orica, Universidad Aut\'onoma de Madrid, Campus de Cantoblanco, Madrid, E-28049, Spain}
%
\affiliation[19]{
Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\affiliation[20]{
Pacific Northwest National Laboratory (PNNL), Richland, WA 99352, USA}
%
\affiliation[21]{
Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%
\affiliation[22]{
Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\affiliation[23]{
Centro de Astropart\'iculas y F\'isica de Altas Energ\'ias (CAPA), Universidad de Zaragoza, Calle Pedro Cerbuna, 12, Zaragoza, E-50009, Spain}
%
\affiliation[24]{
University of the Basque Country (UPV/EHU), Faculty of Chemistry, Manuel de Lardizabal 3, 20018 San Sebastián / Donostia, Spain}
%
\affiliation[25]{
Materials Physics Center. Manuel de Lardizabal 5, 20018 San Sebastián / Donostia, Spain}
%
\affiliation[26]{
Department of Chemistry and Biochemistry, University of Texas at Arlington, Arlington, TX 76019, USA}
%



